The infrared line-emitting regions of T Tauri protoplanetary disks

Mid-infrared molecular line emission detected with the Spitzer Space Telescope is often interpreted using slab models. However, we need to understand the mid-infrared line emission in 2D disk models, such that we gain information about from where the lines are being emitted and under which conditions, such that we gain information about number densities, temperatures, and optical depths in both the radial and vertical directions. In this paper, we introduce a series of 2D thermochemical models of a prototypical T Tauri protoplanetary disk, in order to examine how sensitive the line-emitting regions are to changes in the UV and X-ray fluxes, the disk flaring angle, dust settling, and the dust-to-gas ratio. These all affect the heating of the inner disk, and thus can affect the mid-infrared spectral lines. Using the ProDiMo and FLiTs codes, we produce a series of 2D thermochemical disk models. We find that there is often a significant difference between the gas and dust temperatures in the line emitting regions, and we illustrate that the size of the line emitting regions is relatively robust against changes in the stellar and disk parameters (namely, the UV and X-ray fluxes, the flaring angle, and dust settling). These results demonstrate the potential for localized variations in the line-emitting region to greatly affect the resulting spectra and line fluxes, and the necessity of allowing for such variations in our models.

==> macros.tex <==
\newcommand{\twco}{\cem{^12CO}}
\newcommand{\thco}{\cem{^13CO}}
\newcommand{\cego}{\cem{C^18O}}
\newcommand{\hcn}{\cem{HCN}}
\newcommand{\cn}{\cem{CN}}
\newcommand{\hcop}{\cem{HCO+}}
\newcommand{\pc}{\mathrm{pc}}
\newcommand{\kms}{\ensuremath{\mathrm{km~s}^{-1}}}
\newcommand{\myr}{\ensuremath{\mathrm{Myr}}}
\newcommand{\gyr}{\ensuremath{\mathrm{Gyr}}}
\newcommand{\cm}{\ensuremath{\mathrm{cm}}}
\newcommand{\erg}{\ensuremath{\mathrm{erg}}}
\newcommand{\persec}{\ensuremath{\mathrm{s}^{-1}}}
\newcommand{\mjykms}{\ensuremath{\mathrm{mJy~km~s}^{-1}}}
\newcommand{\mjy}{\ensuremath{\mathrm{mJy}}}
\newcommand{\jy}{\ensuremath{\mathrm{Jy}}}
\newcommand{\jthrtwo}{~\ensuremath{{J=3-2}}}
\newcommand{\jfrthr}{~\ensuremath{{J=4-3}}}
\newcommand{\jsvsx}{~\ensuremath{{J=7-6}}}
\newcommand{\jtwoone}{~\ensuremath{{J=2-1}}}
\newcommand{\msun}{\ensuremath{\mathrm{M}_\odot}}
\newcommand{\rsun}{\ensuremath{\mathrm{R}_\odot}}
\newcommand{\mearth}{\ensuremath{\mathrm{M}_\oplus}}
\newcommand{\mj}{\ensuremath{\mathrm{M}_\mathrm{J}}}
\newcommand{\lsun}{\ensuremath{\mathrm{L}_\odot}}
\newcommand{\mstar}{\ensuremath{M_*}}
\newcommand{\lstar}{\ensuremath{L_*}}
\newcommand{\rstar}{\ensuremath{R_*}}
\newcommand{\mdisk}{\ensuremath{M_\mathrm{disk}}}
\newcommand{\mdust}{\ensuremath{M_\mathrm{dust}}}
\newcommand{\mgas}{\ensuremath{M_\mathrm{gas}}}
\newcommand{\mjup}{\ensuremath{M_\mathrm{Jup}}}
\newcommand{\zetacr}{\ensuremath{\zeta_\mathrm{CR}}}
\newcommand{\au}{\ensuremath{\mathrm{AU}}}
\newcommand{\av}{\ensuremath{\mathrm{A}_V}}
\newcommand{\micron}{\ensuremath{\mu\mathrm{m}}}
\newcommand{\teff}{\ensuremath{T_\mathrm{eff}}}
\newcommand{\kelvin}{\ensuremath{\mathrm{K}}}
\newcommand{\fuv}{\ensuremath{f_\mathrm{UV}}}
\newcommand{\luv}{\ensuremath{L_\mathrm{UV}}}
\newcommand{\puv}{\ensuremath{p_\mathrm{UV}}}
\newcommand{\tline}{\ensuremath{\tau_\mathrm{line}}}
\newcommand{\lxr}{\ensuremath{L_\mathrm{X-ray}}}
\newcommand{\rtaper}{\ensuremath{R_\mathrm{taper}}}
\newcommand{\rin}{\ensuremath{R_\mathrm{in}}}
\newcommand{\rout}{\ensuremath{R_\mathrm{out}}}
\newcommand{\amin}{\ensuremath{a_\mathrm{min}}}
\newcommand{\amax}{\ensuremath{a_\mathrm{max}}}
\newcommand{\apow}{\ensuremath{a_\mathrm{pow}}}
\newcommand{\vsep}{\ensuremath{v_\mathrm{sep}}}
\newcommand{\rv}{\ensuremath{R_V}}
\newcommand{\extinct}{\ensuremath{A_V}}
\newcommand{\tgas}{\ensuremath{T_\mathrm{gas}}}
\newcommand{\tdust}{\ensuremath{T_\mathrm{dust}}}

\newcommand{\jwst}{\mbox{\textit{JWST}}}
\newcommand{\spitzer}{\mbox{\textit{Spitzer}}}
\newcommand{\flits}{\texttt{FLiTs}}
\newcommand{\prodimo}{\texttt{ProDiMo}}

\newcommand{\spica}{\mbox{\textit{SPICA}}}
\newcommand{\herschel}{\mbox{\textit{Herschel}}}
\newcommand{\dali}{\texttt{DALI}}
\newcommand{\elt}{\mbox{ELT}}

\newcommand{\alma}{ALMA}
\newcommand{\twopoppy}{\texttt{two-pop-py}}
\newcommand{\mcmax}{\texttt{MCMax}}

\newcommand{\ngrains}{\ensuremath{N_\mathrm{grains}}}
\newcommand{\nrad}{\ensuremath{N_\mathrm{rad}}}
\newcommand{\ntheta}{\ensuremath{N_\theta}}
\newcommand{\azero}{\ensuremath{a_0}}
\newcommand{\tmax}{\ensuremath{t_\mathrm{max}}}
\newcommand{\alphaturb}{\ensuremath{\alpha_\mathrm{turb}}}
\newcommand{\tstar}{\ensuremath{T_*}}

\newcommand{\chiism}{\ensuremath{\chi_\mathrm{ISM}}}
\newcommand{\fpah}{\ensuremath{f_\mathrm{PAH}}}

\newcommand{\fline}{\ensuremath{F_\mathrm{line}}}

\newcommand{\mr}[1]{\ensuremath{\mathrm{#1}}}  %ensure math / roman font for input

\newcommand{\avgtgas}{\ensuremath{\langle \tgas \rangle}}
\newcommand{\avggasdust}{\ensuremath{\langle \mathrm{g}/\mathrm{d} \rangle}}
\newcommand{\tautwenty}{\ensuremath{\langle \tau _{20~\micron} \rangle}}

==> packages.tex <==
\RequirePackage{txfonts}
\RequirePackage{microtype}
\RequirePackage{graphicx}
\RequirePackage{booktabs}
\RequirePackage{amsmath,amssymb}
\RequirePackage{cleveref}
\RequirePackage{pdfpages}
\RequirePackage{textgreek}


\newcommand*{\rangeto}{\textnormal{\hskip.1em\relax--\hskip.1em\relax}}
\RequirePackage[separate-uncertainty=true,range-units=single,range-phrase=\rangeto,forbid-literal-units=true]{siunitx}



% common astronomical symbols
\let\sun\odot
\let\bh\bullet
\newcommand*{\solarmass}{\si{\solarmass}}
\newcommand*{\solarluminosity}{\si{\solarluminosity}}
% astrophysical units
\DeclareSIUnit\lightspeed{$c$}
\DeclareSIUnit\rydberg{Ry}
\DeclareSIUnit\erg{erg}
\DeclareSIUnit\magnitude{mag}
\DeclareSIUnit\jansky{Jy}
\DeclareSIUnit\gauss{G}
\DeclareSIUnit\h{$h$}
\DeclareSIUnit\hseven{$h$_7}
\DeclareSIUnit\parsec{pc}
\DeclareSIUnit\au{AU}
\DeclareSIUnit\year{yr}
\DeclareSIUnit\solarluminosity{\ensuremath{L_\sun}}
\DeclareSIUnit\solarmass{\ensuremath{M_\sun}}
\DeclareSIUnit\jupitermass{\ensuremath{M_\mathrm{J}}}
\DeclareSIUnit\solarmassinenergy{\ensuremath{M_\sun|c^2}}
\DeclareSIUnit\solarradius{\ensuremath{R_\sun}}

% redeclared units
\DeclareSIUnit\arcsecond{as}
%\DeclareSIUnit\astronomicalunit{AU}
\DeclareSIUnit\clight{\ensuremath c}
% additional unit notations
\DeclareRobustCommand\SIfrac{\@ifstar\astrosym@SIfracplain\astrosym@SIfracparen}
%\newcommand*{\astrosym@SIfracplain}[1]{\begingroup\def\@tempa{#1}\astrosym@@SIfracplain}
%\newcommand*{\astrosym@SIfracparen}[1]{\begingroup\def\@tempa{#1}\astrosym@@SIfracparen}
%\newcommand*{\astrosym@@SIfracplain}[2][]{\frac{\@tempa}{\SI{#1}{#2}}\endgroup}
%\newcommand*{\astrosym@@SIfracparen}[2][]{\biggl(\astrosym@@SIfracplain{#1}{#2}\biggr)}
%\newcommand*{\SIex}[2]{#1\,\si{#2}}
% spectroscopic notation
%\DeclareRobustCommand\specatom{\@ifstar\astrosym@atomforbid\astrosym@atomallow}
%\DeclareRobustCommand\specline{\@ifstar\astrosym@lineforbid\astrosym@lineallow}
%\newcommand*{\astrosym@atomforbid}[2]{\textnormal{[\astrosym@atomallow{#1}{#2}]}}
%\newcommand*{\astrosym@atomallow}[2]{%
%  \textnormal{#1\hskip.1em\relax\textsc{\romannumeral#2}}}
%\newcommand*{\astrosym@lineforbid}[3]{%
%  \textnormal{\astrosym@atomforbid{#1}{#2}\hskip.2em\relax#3}}
%\newcommand*{\astrosym@lineallow}[3]{%
%  \textnormal{\astrosym@atomallow{#1}{#2}\hskip.1em\relax#3}}
% term symbol
%\DeclareRobustCommand\termsym{\@ifstar\astrosym@termodd\astrosym@termeven}
%\newcommand*{\scripts}[5]{\ensuremath{
%  ^{#2\vphantom0}_{#3\vphantom0}\hskip-\scriptspace{#1}
%  ^{#4\vphantom0}_{#5\vphantom0}}}
%\newcommand*{\astrosym@termeven}[3]{\scripts{\textup{#2}}{#1}{}{}{#3}}
%\newcommand*{\astrosym@termodd}[3]{\scripts{\textup{#2}}{#1}{}{\textup o}{#3}}

==> thepreamble.tex <==
\usepackage{lscape}
\usepackage{algorithmic}
\usepackage{subfiles}
%\usepackage{accsupp}
\usepackage{amssymb}
\usepackage{placeins}
\usepackage{pgffor}
\usepackage{morefloats}


\usepackage{graphicx}

\usepackage{xfrac}

%\usepackage{smoothpic} %Blurs edges of images (ie jpegs)

%\RequirePackage[mathcal,text-hat-accent]{euler}






%\defaultfontfeatures{Ligatures=TeX,Numbers=Lining}



%%%%%%%%%%%%%
%Set up plotting
%%%%%%%%%%%%%
\usepackage{tikz}		
	\usepackage{pgfplots,pgfplotstable}
\pgfplotsset{plot coordinates/math parser=false}
\pgfplotsset{compat=1.9}
\usepgfplotslibrary{colormaps}
\usetikzlibrary{spy,shapes.geometric}
	%\usepackage{gnuplot-lua-tikz}
		\usetikzlibrary{plotmarks,positioning,calc,fadings,decorations.pathreplacing,arrows,decorations.markings,patterns, decorations.pathmorphing}
		\usepgfplotslibrary{external}
\makeatletter
\newcommand{\useexternalfile}[1]{%
    \tikzsetnextfilename{#1-pdfout}%
    \input{\tikzexternal@filenameprefix#1.tikz}}
\makeatother
\tikzexternalize%[mode=list and make]
\tikzset{external/system call={pdflatex \tikzexternalcheckshellescape -halt-on-error -interaction=batchmode -jobname "\image" "\texsource"}}

%%%%%%%%%
%
%  If compiling from Terminal, use pdflatex -shell-escape filename
%
%%%%%%%%%

\newlength\figureheight
\newlength\figurewidth

%Make citations in small caps and lower case
%\let\oldcite\cite
%\renewcommand{\cite}[1]{\textsc{\oldcite{#1}}}
%\let\oldcitet\citet
%\renewcommand{\citet}[1]{\textsc{\oldcitet{#1}}}
%\let\oldcitep\citep
%\renewcommand{\citep}[1]{\textsc{\oldcitep{#1}}}

%Colours
%\definecolor{bluecustom}{rgb}{0.254901960784314,0.411764705882353,0.882352941176471}%
%\definecolor{redcustom}{rgb}{0.6,0,0}%
%\definecolor{lightred}{rgb}{0.996,0.898,0.851}%
%\definecolor{greencustom}{rgb}{0,0.5,0}%

\definecolor{bluecustom}{RGB}{72,98,126}%
\definecolor{redcustom}{rgb}{0.55,0,0}%
\definecolor{lightred}{RGB}{247,225,223}%
\definecolor{greencustom}{RGB}{30,77,43}%
\definecolor{blackcustom}{RGB}{1,1,1}

%5-colour diverging scheme - OK to skip 'c' if wanting 4 colours. Needs background for visbility
%\definecolor{rbdivergea}{cmyk}{0,0.88,0.87,0.16}
%\definecolor{rbdivergeb}{cmyk}{0,0.31,0.62,0.01}
%\definecolor{rbdivergec}{cmyk}{0,0,0.25,0}
%\definecolor{rbdiverged}{cmyk}{0.27,0.07,0,0.09}
%\definecolor{rbdivergee}{cmyk}{0.76,0.32,0,0.29}


\definecolor{rbdivergea}{RGB}{202,0,32}
\definecolor{rbdivergeb}{RGB}{244,165,130}
\definecolor{rbdivergec}{RGB}{247,247,247}
\definecolor{rbdiverged}{RGB}{146,197,222}
\definecolor{rbdivergee}{RGB}{5,113,176}




%5-color qualitative scheme
%\definecolor{rbquala}{cmyk}{0,0.89,0.88,0.11} %red
%\definecolor{rbqualb}{cmyk}{0.70,0.32,0,0.28} %blue
%\definecolor{rbqualc}{cmyk}{0.56,0,0.58,0.31} %green
%\definecolor{rbquald}{cmyk}{0.07,0.52,0,0.36} %purple
%\definecolor{rbquale}{cmyk}{0,0.50,100,0} %orange

\definecolor{rbquala}{RGB}{228,26,28}
\definecolor{rbqualb}{RGB}{55,126,184}
\definecolor{rbqualc}{RGB}{77,175,74}
\definecolor{rbquald}{RGB}{152,78,163}
\definecolor{rbquale}{RGB}{255,127,0}



\pgfplotsset{colormap={bonecmap}{[1pt] rgb(0pt)=(0,0,0.0416667); rgb(2pt)=(0.194444,0.194444,0.319444); rgb(5pt)=(0.486111,0.611111,0.611111); rgb(9pt)=(1,1,1)}}



%\pgfplotsset{colormap={bandw}{gray(0cm)=(0.00); gray(1cm)=(0.15); gray(9cm)=(0.92); gray(10cm)=(0.96)}}

%\pgfplotsset{colormap={bandw}{cmyk(0cm)=(0,0.03,0,0.03); cmyk(1cm)=(0.16,0.11,0,0.12); cmyk(2cm)=(0.50,0.18,0,0.19); cmyk(3cm)=(0.82,0.06,0,0.40); cmyk(4cm)=(0.99,0,0.18,0.58)}}



\pgfplotsset{colormap={bandw}{[1pt]
rgb(0pt)=(0.192157,0.211765,0.584314);
rgb(1pt)=(0.270588,0.458824,0.705882);
rgb(2pt)=(0.454902,0.678431,0.819608);
rgb(3pt)=(0.670588,0.850980,0.913725);
rgb(4pt)=(0.878431,0.952941,0.972549);
rgb(5pt)=(1.000000,1.000000,0.749020);
rgb(6pt)=(0.996078,0.878431,0.564706);
rgb(7pt)=(0.992157,0.682353,0.380392);
rgb(8pt)=(0.956863,0.427451,0.262745);
rgb(9pt)=(0.843137,0.188235,0.152941);
rgb(10pt)=(0.647059,0.00000,0.149020)}}



\pgfplotsset{colormap={bandwinvert}{[1pt]
rgb(0pt)=(0.647059,0.00000,0.149020);
rgb(1pt)=(0.843137,0.188235,0.152941);
rgb(2pt)=(0.956863,0.427451,0.262745);
rgb(3pt)=(0.992157,0.682353,0.380392);
rgb(4pt)=(0.996078,0.878431,0.564706);
rgb(5pt)=(1.000000,1.000000,0.749020);
rgb(6pt)=(0.878431,0.952941,0.972549);
rgb(7pt)=(0.670588,0.850980,0.913725);
rgb(8pt)=(0.454902,0.678431,0.819608);
rgb(9pt)=(0.270588,0.458824,0.705882);
rgb(10pt)=(0.192157,0.211765,0.584314)}}








%\pgfplotsset{colormap={randb}{cmyk(0cm)=(0.0885,0.9557,0.7590,0.2444); cmyk(1cm)=(0.0488,0.0134,0.2515,0); cmyk(2cm)=(0.9332,0.8412,0.0066,0.0207)}}

%\pgfplotsset{colormap={randb}{
%cmyk(0cm)=(0.35,1,0.70,0);
%cmyk(1cm)=(0.15,0.80,0.75,0);
%cmyk(2cm)=(0.3,0.57,0.63,0);
%cmyk(3cm)=(0,0.35,0.55,0);
%cmyk(4cm)=(0,0.12,0.40,0);
%cmyk(5cm)=(0,0,0.25,0);
%cmyk(6cm)=(0.12,0,0,0);
%cmyk(7cm)=(0.33,0.03,0,0);
%cmyk(8cm)=(0.55,0.15,0,0);
%cmyk(9cm)=(0.75,0.37,0,0);
%cmyk(10cm)=(0.85,0.70,0,0)
%}}






%\pgfplotsset{colormap={bandwextreme}{cmyk(0cm)=(0,0.03,0,0.03); cmyk(2cm)=(0.05,0.06,0,0.06); cmyk(6cm)=(0.16,0.11,0,0.12); cmyk(8cm)=(0.50,0.18,0,0.19); cmyk(10cm)=(0.82,0.06,0,0.40); cmyk(16cm)=(0.99,0,0.18,0.58)}}







%\pgfplotsset{colormap={orangetored}{ rgb255(0cm)=(254,229,217); rgb255(1cm)=(252,174,145); rgb255(2cm)=(251,106,74);  rgb255(3cm)=(222,45,38); rgb255(4cm)=(165,15,21); rgb255(5cm)=(100,10,16)}}
%\pgfplotsset{colormap={orangetoredlogmodelconvergence}{ rgb255(0cm)=(254,229,217); rgb255(2cm)=(252,174,145); rgb255(4cm)=(251,106,74);  rgb255(10cm)=(222,45,38); rgb255(30cm)=(165,15,21); rgb255(60cm)=(100,10,16)}}

%\pgfplotsset{colormap={orangetored}{ cmyk(0cm)=(0,0,0.17,0); cmyk(1cm)=(0,0.15,0.44,0); cmyk(2cm)=(0,0.40,0.84,0);  cmyk(3cm)=(0,0.56,0.94,0.15); cmyk(4cm)=(0,0.66,0.97,0.40); cmyk(5cm)=(0,0.63,1,0.78)}}
%\pgfplotsset{colormap={orangetoredlogmodelconvergence}{ cmyk(0cm)=(0,0,0.17,0); cmyk(2cm)=(0,0.15,0.44,0); cmyk(4cm)=(0,0.40,0.84,0);  cmyk(10cm)=(0,0.56,0.94,0.15); cmyk(30cm)=(0,0.66,0.97,0.40); cmyk(60cm)=(0,0.63,1,0.78)}}

%\pgfplotsset{colormap={orangetored}{
%rgb(0pt)=(1,1,0.898039);
%rgb(1pt)=(1,0.968627,0.737255);
%rgb(2pt)=(0.996078,0.890196,0.568627);
%rgb(3pt)=(0.996078,0.768627,0.309804);
%rgb(4pt)=(0.996078,0.6,0.160784);
%rgb(5pt)=(0.92549,0.439216,0.0784314);
%rgb(6pt)=(0.8,0.298039,0.00784314);
%rgb(7pt)=(0.6,0.203922,0.0156863);
%rgb(8pt)=(0.4,0.145098,0.0235294)}}

%\pgfplotsset{colormap={orangetoredlogmodelconvergence}{
%rgb(0pt)=(1,1,0.898039);
%rgb(2pt)=(1,0.968627,0.737255);
%rgb(4pt)=(0.996078,0.890196,0.568627);
%rgb(12pt)=(0.996078,0.768627,0.309804);
%rgb(20pt)=(0.996078,0.6,0.160784);
%rgb(28pt)=(0.92549,0.439216,0.0784314);
%rgb(38pt)=(0.8,0.298039,0.00784314);
%rgb(46pt)=(0.6,0.203922,0.0156863);
%rgb(60pt)=(0.4,0.145098,0.0235294)}}



%NEW ORANGETORED SAME AS PUBUGN
\pgfplotsset{colormap={orangetored}{
rgb(0pt)=(1,0.968627,0.984314);
rgb(1pt)=(0.92549,0.886275,0.941176);
rgb(2pt)=(0.815686,0.819608,0.901961);
rgb(3pt)=(0.65098,0.741176,0.858824);
rgb(4pt)=(0.403922,0.662745,0.811765);
rgb(5pt)=(0.211765,0.564706,0.752941);
rgb(6pt)=(0.00784314,0.505882,0.541176);
rgb(7pt)=(0.00392157,0.423529,0.34902);
rgb(8pt)=(0.00392157,0.27451,0.211765)}}


\pgfplotsset{colormap={orangetoredlogmodelconvergence}{
rgb(0pt)=(1,0.968627,0.984314);
rgb(2pt)=(0.92549,0.886275,0.941176);
rgb(4pt)=(0.815686,0.819608,0.901961);
rgb(12pt)=(0.65098,0.741176,0.858824);
rgb(20pt)=(0.403922,0.662745,0.811765);
rgb(28pt)=(0.211765,0.564706,0.752941);
rgb(38pt)=(0.00784314,0.505882,0.541176);
rgb(46pt)=(0.00392157,0.423529,0.34902);
rgb(60pt)=(0.00392157,0.27451,0.211765)}}




\pgfplotsset{colormap={pubugn}{
rgb(0pt)=(1,0.968627,0.984314);
rgb(1pt)=(0.92549,0.886275,0.941176);
rgb(2pt)=(0.815686,0.819608,0.901961);
rgb(3pt)=(0.65098,0.741176,0.858824);
rgb(4pt)=(0.403922,0.662745,0.811765);
rgb(5pt)=(0.211765,0.564706,0.752941);
rgb(6pt)=(0.00784314,0.505882,0.541176);
rgb(7pt)=(0.00392157,0.423529,0.34902);
rgb(8pt)=(0.00392157,0.27451,0.211765)}}


%Use interp or flat shaders for PGF plots

\newcommand{\shadertype}{interp}


%\pgfdeclareplotmark{hexagon}
%{%
%  \pgfpathmoveto{\pgfqpoint{0pt}{1.1547\pgfplotmarksize}}
%  \pgfpathlineto{\pgfqpointpolar{150}{1.1547\pgfplotmarksize}}
%  \pgfpathlineto{\pgfqpointpolar{210}{1.1547\pgfplotmarksize}}
%  \pgfpathlineto{\pgfqpointpolar{270}{1.1547\pgfplotmarksize}}
%  \pgfpathlineto{\pgfqpointpolar{330}{1.1547\pgfplotmarksize}}
%  \pgfpathlineto{\pgfqpointpolar{30}{1.1547\pgfplotmarksize}}
%  \pgfpathclose
%\pgfusepathqfill
%}
%
\pgfdeclareplotmark{hexagon}
{%
  \pgfpathmoveto{\pgfqpointpolar{90}{0.0067857143\figurewidth}}  % 10% enlargement, 70-hexagon resolution. 0.95/(2*70) = 0.0067857143
  \pgfpathlineto{\pgfqpointpolar{150}{0.0067857143\figurewidth}}
  \pgfpathlineto{\pgfqpointpolar{210}{0.0067857143\figurewidth}}
  \pgfpathlineto{\pgfqpointpolar{270}{0.0067857143\figurewidth}}
  \pgfpathlineto{\pgfqpointpolar{330}{0.0067857143\figurewidth}}
  \pgfpathlineto{\pgfqpointpolar{30}{0.0067857143\figurewidth}}
  \pgfpathclose
\pgfusepathqfill
}


%\pgfdeclareplotmark{hexagon}
%{%
%\node[regular polygon, regular polygon sides=6, draw,
%     outer sep=0,inner sep=0,minimum size=0.007142857\figurewidth,fill] at (0,0) {};
%}






\pgfdeclareplotmark{hexagononefifty}
{%
  \pgfpathmoveto{\pgfqpoint{0pt}{1\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{150}{1\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{210}{1\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{270}{1\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{330}{1\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{30}{1\pgfplotmarksize}}
  \pgfpathclose
\pgfusepathqfill
}





%%%
% preamble from BD geometry paper
%%%










\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}

\usepackage{hyperref}


\usepackage{booktabs}

\usepackage{placeins}%
\usepackage{afterpage}% http://ctan.org/pkg/afterpage
\usepackage{float}% http://ctan.org/pkg/float
\usepackage[flushleft]{threeparttable}
\usepackage{tikz,pgfplots}


%\mhchemoptions{textfontcommand=\fontfamily{hlh}\selectfont}
%\mhchemoptions{mathfontcommand=\fontfamily{hlh}\selectfont\text}

\usepackage{csvsimple}


\sisetup{%
	output-decimal-marker={.},
	group-separator={ },
	per-mode=fraction,
	group-digits=integer, %true,false,integer, or decimal
	table-number-alignment = right,
	table-parse-only = true % do not use S column type to align numbers	
}

% footnote without marker / counter
\newcommand\blfootnote[1]{%
	\begingroup
	\renewcommand\thefootnote{}\footnote{#1}%
	\addtocounter{footnote}{-1}%
	\endgroup
}


